Attentive Explanations: Justifying Decisions and Pointing to the Evidence (Extended Abstract)

Deep models are the defacto standard in visual decision problems due to their impressive performance on a wide array of visual tasks. On the other hand, their opaqueness has led to a surge of interest in explainable systems. In this work, we emphasize the importance of model explanation in various forms such as visual pointing and textual justification. The lack of data with justification annotations is one of the bottlenecks of generating multimodal explanations. Thus, we propose two large-scale datasets with annotations that visually and textually justify a classification decision for various activities, i.e. ACT-X, and for question answering, i.e. VQA-X. We also introduce a multimodal methodology for generating visual and textual explanations simultaneously. We quantitatively show that training with the textual explanations not only yields better textual justification models, but also models that better localize the evidence that support their decision.

==> datasettable.tex <==
{
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[tb]
\begin{center}
\small
\begin{tabular}{l l l l|rrrrr r|rrrrr r}
\toprule
&Train-&Att.&Answer& \multicolumn{6}{c|}{VQA-X} & \multicolumn{6}{c}{ACT-X} \\
&ing &  for & Condi-& \multicolumn{5}{c}{Automatic evaluation} & \multicolumn{1}{c|}{Human} &\multicolumn{5}{c}{Automatic evaluation} & \multicolumn{1}{c}{Human}\\
Approach &  Data & Expl. &  tioning & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{C} &\multicolumn{1}{c}{S} &\multicolumn{1}{c|}{eval} & \multicolumn{1}{c}{B} & \multicolumn{1}{c}{M} & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{C} &\multicolumn{1}{c}{S} &\multicolumn{1}{c}{eval}  \\
\midrule
\cite{hendricks16eccv} & Desc. & No & Yes &\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&\multicolumn{1}{c}{--}&12.9 & 15.9  & 39.0 & 12.4 & 12.0 &7.6  \\ %generation_result.json
Ours on Descriptions & Desc. & Yes & Yes & 8.1 & 14.3  & 28.3  & 34.3 & 11.2 &24.0 & 6.9  & 12.9 & 28.3 & 20.3 & 7.3&18.0  \\ %des_test_results_15000.json
\midrule
Captioning Model & Expl. & Yes & No &17.1 &16.0 &40.4 &43.6 &7.3 &19.2 &20.7 &18.8 &44.3 &40.7 &11.3&20.4 \\ %cap_test_results_17500.json
Ours w/o Exp-Attention & Expl. & No & Yes &25.1 &20.5 &48.7 &74.2 &11.6 &34.4& 16.9 &17.0 &42.0&33.3 &10.6 &17.6  \\ %noatt_test_results_32500.json
Ours & Expl. & Yes & Yes &25.3 &20.9  &49.8 &72.1 &12.1 & 33.6 & 24.5 &21.5 &46.9 &58.7 &16.0 & 26.4  \\ %ours_test_results_22500.json
Finetuned & Expl. & Yes & Yes &27.1 &20.9  &49.9 &77.2 &11.8 & -- & -- & -- & -- & -- & -- & --  \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Evaluation of Textual Justifications. Evaluated automatic metrics: BLEU-4 (B), METEOR (M), ROUGE (R), CIDEr (C) and SPICE (S). Reference sentence for human and automatic evaluation is always an explanation. All in \%.  Our proposed model compares favorably to baselines.}
\vspace{-4mm}
\label{tbl:generation_automatic}
\end{center}
\end{table*}
}



==> qualitative_fig.tex <==
\begin{figure*}[h]
\begin{center}
  \includegraphics[width=\linewidth]{images/supp_sameqa_diffimg}
\end{center}
\caption{VQA-X results with the same question/answer pair. We select results with the same question and answer pair with two different images and show that although the QA pairs are the same, for different images our model generates different explanations (Answers are correctly predicted). VQA-ATT denotes attention maps used for predicting answers and EXP-ATT denotes attention maps used for generating the corresponding justifications.}
\label{fig:VQAqualitative-sameQA}
\end{figure*}

\begin{figure*}[h]
\begin{center}
  \includegraphics[width=\linewidth]{images/supp_sameimg_diffqa}
\end{center}
\caption{VQA-X results with same image and different questions. We select results with the same image and different Q/A pairs and show that although the images are the same, our model is able to answer the questions differently and generate a different explanation accordingly (Answers are correctly predicted). VQA-ATT denotes attention maps used for predicting answers and EXP-ATT denotes attention maps used for generating the corresponding justifications.}
\label{fig:VQAqualitative-sameimage}
\end{figure*}

\begin{figure*}[h]
\begin{center}
 \includegraphics[width=\linewidth]{images/supp_sameact_diffimg}
  %\includegraphics[width=\linewidth]{ACT_similar_activities}
\end{center}
\caption{ACT-X results with similar activities. Figure on the left: We show results with fine-grained activities all related to windsurfing, kayaking, canoeing and observe that both the fine-grained activities are correctly predicted and the explanations match the activity and the image. Figure on the right: We show results with fine-grained activities all related to bicycling and observe that both the fine-grained activities are correctly predicted and the explanations match the activity and the image. ACT-ATT denotes attention maps used for predicting answers and EXP-ATT denotes attention maps used for generating the corresponding justifications.}
\label{fig:ACTqualitative:similar:activity}
\end{figure*}

\begin{figure*}[h]
\begin{center}
 \includegraphics[width=\linewidth]{images/vqa_right_wrong}
  %\includegraphics[width=\linewidth]{ACT_similar_activities}
\end{center}
\caption{VQA-X results. GT denotes ground-truth answer while P indicates actual prediction made by the model. Figure on the left: We show various qualitative results with correctly predicted answer and observe that the explanation justifies the answer accordingly. Figure on the right: We show results with incorrectly predicted answer and observe that although the answer is incorrect, our model can provide visual and textual explanations on why the model might be failing in those cases.}
\label{fig:VQAqualitative:correct_incorrect}
\end{figure*}

\begin{figure*}[h]
\begin{center}
 \includegraphics[width=\linewidth]{images/activity_right_wrong}
  %\includegraphics[width=\linewidth]{ACT_similar_activities}
\end{center}
\caption{ACT-X results. GT denotes ground-truth answer while P indicates actual prediction made by the model. Figure on the left: We show various qualitative results with correctly predicted answer and observe that the explanation justifies the answer accordingly. Figure on the right: We show results with incorrectly predicted answer and observe that although the answer is incorrect, our model can provide visual and textual explanations on why the model might be failing in those cases.}
\label{fig:ACTqualitative:correct_incorrect}
\end{figure*}
